A Fast, Compact, Accurate Model for Language Identification of Codemixed Text

We address fine-grained multilingual language identification: providing a language code for every token in a sentence, including codemixed text containing multiple languages. Such text is prevalent online, in documents, social media, and message boards. We show that a feed-forward network with a simple globally constrained decoder can accurately and rapidly label both codemixed and monolingual text in 100 languages and 100 language pairs. This model outperforms previously published multilingual approaches in terms of both accuracy and speed, yielding an 800x speed-up and a 19.5% averaged absolute gain on three codemixed datasets. It furthermore outperforms several benchmark systems on monolingual language identification.

==> intro_old.tex <==
\section{Introduction}
% * <yuanzh@csail.mit.edu> 2018-02-09T00:06:11.931Z:
% 
% Comments from SAFT:
% 1. Over 50 per cent of the world’s population function in two or more languages on a daily basis. Multilingualism, not monolingualism, is the norm. Good to find a scientific source. https://www.britishcouncil.org/voices-magazine/few-myths-about-speakers-multiple-languages
% DONE % 2. Mention data release in abstract and intro.
% 3. I think you can do a better job describing token-level LangID vs doc-level LangID and how data for doc-level is easier to get and plentiful and the task is much easier, while token-level is harder but really needed. (perhaps also in task formulation)
% PARTIALLY DONE. % 4. High-level comment: right now the paper reads a bit like a system description. What is your research hypothesis and what are the scientific take-aways? Most of the info is in the paper, but I would probably restructure the paper with these questions in mind. IMHO, your contributions are: (a) New dataset/task that is well motivated and explained (b) Techniques for dealing with a big mismatch between training and test conditions: Decoding constraints Various features,  Selective dropout, etc 
% With the previous comment in mind, it might make sense to build your model up step-by-step, showing results as you go. Right now, you start with a fairly dry modeling section and then have a very long results/analysis section. Interweaving the two might make for a better read. Just an idea...
% MOSTLY DONE BUT WE NEED TO SHOW HOW MUCH OUR MODEL STOMPS ON THE PERFORMANCE OF PREVIOUS WORK % 5. What contributions I see: (a) New corpus and task definition (ps the task is high importance in modern world) (not clear to me how new the task is, given the existence of per-character langid models?) (b) Accuracy: totally supersedes old task: per-token model does harder thing but ps actually does better at per-sentence too (c) Global constraints decoding mechanism (d) speed? (as mentioned above, I’m not sure)
% 
% TODO ADDED % 6. Abstract: include evaluation statistics?
% 7. Introduction: What gaps are you addressing that aren’t already addressed in the Language Identification in Code-Switched Data? 
% REMOVED % 8. Introduction: lyrics to a pop song
% DONE % 9. Introduction: Can you fit examples into the Introduction of each thing you mention (English-Hindo code-mixing, Korean-English code-mixing, and social media examples are missing) 
% 

Language identification of monolingual text is a practical, well-studied problem \citep{Hughes:2006,Baldwin:2010,Lui:2012,King:2013}, but language identification for codemixed text has received considerably less attention. The proceedings of the shared tasks on Language Identification in Code-Switched Data \citep{solorio-EtAl:2014:CodeSwitch,molina-EtAl:2016:W16-58} cover much of the efforts so far. These have largely aimed at identifying larger language spans in longer documents \citep{Lui:2014} or estimating the overall proportions of different languages in a text \citep{Lui:2014,Kocmi:2017}. In this paper, we address the problem of fine-grained (token-level) language identification, which is directly useful for many multilingual downstream tasks, including syntactic analysis, machine translation and dialog systems.

Codemixing occurs in both documents and short queries. It can involve switches within and across constituents, as seen in the following English-Spanish and English-Hindi examples.

%\ex. \dashuline{lo mejor de todas esas super bowl es michael jackson} \uline{i love you king}\\
%     {\it The best of all those superbowls is Michael Jackson; I love you, king.}\\

%\ex. \dashuline{d\'ia de los muertos} \uline{is remembering the dead not visiting them}\\
%	{\it The Day of the Dead is remembering the dead, not visiting them.}

\ex. \label{ex:intramix} \dashuline{dame} [$_{NP}$ \dashuline{ese} \uline{book that you told me about}]\\
	{\it Give me this book that you told me about.}
    
%\ex. \label{ex:intermix} [$_{NP}$ \dashuline{aapni} \uline{photo}] [$_{VP}$ \uline{send} \dashuline{karo}]\\
\ex. \label{ex:intermix} [$_{NP}$ \dashuline{aapni} \uline{photo}] [$_{VP}$ \dashuline{bhej do}]\\
     {\it Send your photo.}

%\ex. \dashuline{dame ese} \uline{book that you told me about}\\
%	{\it Give me this book that you told me about.}
    
%\ex. \dashuline{aapni} \uline{photo send} \dashuline{karo}\\
%     {\it Send your photo.}

\noindent
\ref{ex:intramix} shows the \textbf{intra-mix} codemixing pattern, in which a sentence starts in one language and has a single switch until the end. \ref{ex:intermix} gives the \textbf{inter-mix} pattern, in which the languages mix throughout the sequence. Often, one language is dominant in \textit{inter-mix} utterances.

Codemixed text often shows up in social media contexts, and compounding the problem of language identification are factors like informality of the lexicon, mispellings, transliteration, and abbreviation \citep{Baldwin:2013}. Consider this real-world mixed French and Arabic segment:
\novocalize
\ex. \dashuline{cv bien} \uline{hmd w enti}\\
     \dashuline{ça va bien} \uline{\textbf{al}h\textbf{a}md\textbf{ullilah} w\textbf{a} enti}\\
     \dashuline{ça va bien} \uline{\RL{al.hmd al-ll_ahi wAnt}}\\
 	{\it It's going well, thank God, and you?}    

%\exg. \dashuline{cv} \dashuline{bien} \uline{hmd} \uline{w} \uline{enti}\\
%     \dashuline{ça va} \dashuline{bien} \uline{\textbf{al}h\textbf{a}md\textbf{ullilah}} %\uline{w\textbf{a}} \uline{enti}\\
%     \dashuline{ça va bien} \uline{\RL{al.hmd al-ll_ahi wAnt}}\\
% 	{\it It's going well, thank God, and you?}    


\noindent
This example shows codemixed text that has undergone transliteration, abbreviation, and diacritic removal. The amount of such textual data in the wild is steadily increasing, along with the need to identify and handle it. \citet{rijhwani-EtAl:2017:Long} estimate that 3.5\% of all tweets are code-mixed. In some regions, particularly in India, codemixing between Hindi and English is commonplace if not the norm, with as much as 17\% of Indian Facebook posts being code-mixed \citep{bali-EtAl:2014:CodeSwitch}. 

%For example, a webpage containing lyrics to a pop song in the original Korean along with its English translation; or, a query to a home assistant device asking for a particular song, "$play$ $despacito$."

%We use language identification very often as a first step in natural language understanding tasks before applying language-specific models for syntactic parsing, tagging, or chunking. We use language identification in gathering training data for language modeling or machine translation (Uszkoreit et al., 2010), or as part of a web browsing experience detecting that a user has visited a page in a foreign language so as to offer a translation. We use it as a precursor to applying the right text-to-speech models to make online text accessible to the visually impaired.


As the above examples demonstrate, fine-grained language identification is a hard task---one made even harder because mismatches between distributions for training and evaluation data are the norm, not the exception. To better evaluate models for the task, we release a corpus of per-token language identification labels on 30k sentences (386k tokens). We combine training on such labeled data with synthetic examples to produced fast and accurate models that generalize well. Our model (\mname) labels every token with simple and efficient feed-forward classifiers; their output is then combined for constrained prediction of language pairs for the entire sentence with a simple decoding method using global constraints. The latter is key to maintaining high-quality predictions on monolingual texts as well as codemixed ones. We furthermore show how selective, blocked dropout enables mixing of character and word-level features in a single model without the latter overwhelming the former. (robust to short queries, informal texts misspelled words)

%As the above examples demonstrate, fine-grained language identification is a hard task---one made even harder because mismatches between distributions for training and evaluation data are the norm, not the exception. To better evaluate models for the task, we release a corpus of per-token language identification labels on 30k sentences (386k tokens). We combine training on such labeled data with synthetic examples to produced fast and accurate models that generalize well. Our model (\mname) labels every token with simple and efficient feed-forward classifiers; their output is then combined for constrained prediction of language pairs for the entire sentence with a simple decoding method using global constraints. The latter is key to maintaining high-quality predictions on monolingual texts as well as codemixed ones. We furthermore show how selective, blocked dropout enables mixing of character and word-level features in a single model without the latter overwhelming the former.

%I think you can do a better job describing token-level LangID vs doc-level LangID and how data for doc-level is easier to get and plentiful and the task is much easier, while token-level is harder but really needed.

\todo{Add sentences with headline numbers that highlight awesomeness of the models.}

\todo{Should we say something in the intro about the challenge (and importance) of getting fine-grained langid annotations?}


% * <yuanzh@csail.mit.edu> 2018-02-02T18:36:01.387Z:
% 
% We can summarize our contribution from two aspects: dataset and modelling
% 
% ^.


% The evolution of social media texts such as blogs, micro-blogs (e.g., Twitter), WhatsApp, and chats (e.g., Facebook messages) has created many new opportunities for information access and language technology, but also many new challenges, making it one of the prime present-day research areas. Non-English speakers, especially Indians, do not always use Unicode to write something in social media in ILs. Instead, they use phonetic typing/ roman script/ transliteration and frequently insert English words or phrases through code-mixing and anglicisms (see the following example [1]), and often mix multiple languages to express their thoughts. While it is clear that English still is the principal language for social media communications, there is a growing need to develop technologies for other languages, including Indian languages. India is home to several hundred languages. Language diversity and dialect changes instigate frequent code-mixing in India. Hence, Indians are multi-lingual by adaptation and necessity, and frequently change and mix languages in social media contexts, which poses additional difficulties for automatic Indian social media text processing. Part-of-speech (POS) tagging is an essential prerequisite for any kind of NLP applications. This year we will continue the last year’s POS tagging shared-task on three widely spoken Indian languages (Hindi, Bengali, and Telugu), mixed with English.
% TOOL CONTEST ON POS TAGGING FOR CODE-MIXED INDIAN SOCIAL MEDIA (FACEBOOK, TWITTER, AND WHATSAPP) TEXT
% Part-of-Speech Tagging for Code-Mixed English-Hindi Twitter and Facebook Chat Messages



==> intro_yuan.tex <==
\comment{zhangyua}{On the high level, I feel the current intro doesn't present a consistent and clear story about the paper. For example, the second paragraph introduces two types of codemixing but it doesn't really help explaining the challenges in our task and our contributions in the paper. I draft a new intro below focusing on presenting the storyline I would like to have in the intro. See comments at the beginning of each paragraph.}
%\comment{zhangyua}{I have a concern that we mentioned all these challenges here but this paper doesn't explicitly address them.}
%\todo{1. emphasize token-level LangID task is harder but really needed, and annotations is also harder to get. 2. emphasize our contribution includes two parts: data and model}
% ``send'' to ``bhej'' so Hindi is dominant

\section{Introduction}
% Doc-level Lang ID has been well studied, but token level is not.
Language identification of monolingual text is a practical, well-studied problem \citep{Hughes:2006,Baldwin:2010,Lui:2012,King:2013}, but language identification for codemixed text has received much less attention. The proceedings of the shared tasks on Language Identification in Code-Switched Data \citep{solorio-EtAl:2014:CodeSwitch,molina-EtAl:2016:W16-58} cover much of the efforts so far. Previous work has largely aimed at identifying larger language spans in longer documents \citep{Lui:2014} or estimating the proportions of multiple languages in a text \citep{Lui:2014,Kocmi:2017}. 

% Token-level Lang ID is useful for many tasks
Most current language identification models break down in the presence of multilingual text, which is increasingly prevalent online, in documents, search queries, tweets, and message boards. In this paper, we address the problem of fine-grained (token-level) language identification, which is directly useful for many multilingual downstream tasks, including syntactic analysis, machine translation and dialog systems. 

Consider a real-world query \textit{Translate Apfel to English}, where the user wants to translate the German word \textit{Apfel} (meaning \textit{apple}) to English. An assistant system is likely to fail on this query if it treats the whole query as a single language, either English or German. However, per-token language labels would allow the system to correctly process this query. The amount of codemixed data in the world is steadily increasing, along with the need to identify and handle it on the token-level.  \citet{rijhwani-EtAl:2017:Long} estimate that 3.5\% of all tweets are code-mixed. In some regions, particularly in India, codemixing between Hindi and English is commonplace if not the norm, with as much as 17\% of Indian Facebook posts being code-mixed \citep{bali-EtAl:2014:CodeSwitch}. 

\comment{riesa: I like this; just a couple comments: Whenever we say "query" I think we need to say search query or assistant query. Outside of google it is not clear. I also am not sure that [translate apfel to english] is going to be the best example just because it works today in google search. Maybe there is another example we can use without the [translate] directive keyword. I'll try to think about this.} 

\comment{riesa: I think the intro might be becoming a little too long but it could be just all the inline comments we have written in here.}

\comment{zhangyua}{agreed. There are also some redundant pieces we can remove. FWIW if we want to interweave related work intro, it does make sense to become a little longer than a regular one.}

\comment{riesa: In addition to the fr/ar-En example below, I think it would be good to keep at least one of the simpler en-es examples that were in here before. It is really simple/easy to digest for the reader to help understand exactly what the inputs/outputs are for this problem.}

% Token-level Lang ID is challenging: 1. annotations are hard to obtain 2. code switching happens a lot in short queries and informal texts
Despite the usefulness of token-level language labels, the token-level language ID tasks presents new challenges comparing to sentence-level language ID. First, unlike sentence-level language labels, per-token labels do not typically available from the metadata of text sources. Instead, we need native speakers to annotate codemixed texts, and it is infeasible to obtain annotations for tens or hundreds of languages. Second, code switching phenomenon often shows up in social media contexts, compounding challenges like informality of the lexicon, mispellings, transliteration, and abbreviation \citep{Baldwin:2013}. Consider this real-world mixed French and Arabic segment:
\novocalize
\ex. \dashuline{cv bien} \uline{hmd w enti}\\
     \dashuline{ça va bien} \uline{\textbf{al}h\textbf{a}md\textbf{ullilah} w\textbf{a} enti}\\
     \dashuline{ça va bien} \uline{\RL{al.hmd al-ll_ahi wAnt}}\\
 	{\it It's going well, thank God, and you?}     

\noindent
This example shows codemixed text that has undergone transliteration, abbreviation, and diacritic removal. It becomes a desiderata for a language ID model to be robust to these surface variations.
\comment{zhangyua}{I have a concern that we mentioned all these challenges here but this paper doesn't explicitly address them.}

\comment{riesa}{I think it's important to note properties of text in which most codemixed data is found. We can add an aside that is beyond the scope of this paper to address them directly but it is important to convey that they serve to compound the problem of language identification especially because there is an unconscious bias in the community that language id has been solved. Certainly it has not been solved for short informal texts and there are a lot of interesting factors at play.}

% In this paper we propose to tackle problem from two orthogonal directions.
% Dataset description
In this paper, we propose to tackle these challenges from two orthogonal directions: data collections and modeling techniques. Our first line of contributions focus on codemixed data collections. We release a corpus of per-token language identification labels on 30k real-word codemixed sentences (386k tokens). This corpus covers three languages (Spanish, Hindi and Indonesian) that commonly have code mixing with English. This corpus serves as both a new training set and a new benchmark for token-level language ID on codemixed text. To generalize our model to 110 languages, we further expand our training data with synthetic examples, generated based on linguistic patterns we found on real-world codemixed texts.

% Modeling description
As the second line of our contributions, we propose \mname, our language ID model for \tb{C}ode\tb{M}i\tb{X}ed text that is fast and accurate. \mname ~labels every token with simple and efficient feed-forward classifiers; their output is then combined for constrained prediction of language pairs for the entire sentence with a simple decoding method using global constraints. The latter is key to maintaining high-quality predictions on monolingual texts as well as codemixed ones. We furthermore show how selective, blocked dropout enables mixing of character and word-level features in a single model without the latter overwhelming the former. This dropout method effectively help the model to be more robust on informal texts, which we will show empirically.


% Summary of results
We evaluate our approach on three codemixed benchmarks covering ten languages, and a monolingual test set including 54 languages. Our model consistently outperforms state-of-the-art, RNN-based language ID models, obtaining a $>$29\% absolute gain on the codemixed benchmarks and a $>$3\% absolute gain (60\% error reduction) on the monolingual corpus. We also demonstrate a resource-friendly variant of our model that saves memory usage from 30M to 0.9M, with only 3.3\% drop on performance. Our model processes inputs at 206k characters per second, which is about 800x faster than existing token-level models. Finally we also provide  analysis on impact of our codemixed datasets and how our techniques help model perform well on short queries and informal texts.

